Information-Flow Matting

We present a novel, purely affinity-based natural image matting algorithm. Our method relies on carefully defined pixel-to-pixel connections that enable effective use of information available in the image. We control the information flow from the known-opacity regions into the unknown region, as well as within the unknown region itself, by utilizing multiple definitions of pixel affinities. Among other forms of information flow, we introduce color-mixture flow, which builds upon local linear embedding and effectively encapsulates the relation between different pixel opacities. Our resulting novel linear system formulation can be solved in closed-form and is robust against several fundamental challenges of natural matting such as holes and remote intricate structures. While our method is primarily designed as a standalone matting tool, we show that it can also be used for regularizing mattes obtained by sampling-based methods. The formulation is also extended to layer color estimation and we show that the use of multiple channels of flow increases the layer color quality. We also demonstrate our performance in green-screen keying and analyze the characteristics of the utilized affinities.

==> images/ablation.tex <==

\begin{table}[t]
\caption{
    Performance decrease when one of the information flows is omitted in the linear system formulation.
    The training dataset \cite{alphabenchmark} of 27 images and 2 trimaps per image (S and L) was used for this comparison.
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
\rowcolors{2}{gray!25}{}
\begin{tabular}{
!{\color{gray!25}\vrule} 
l
!{\color{gray!25}\vrule} 
c 
!{\color{gray!25}\vrule}
c c 
!{\color{gray!25}\vrule} 
!{\color{gray!25}\vrule} 
c 
!{\color{gray!25}\vrule}
c c
!{\color{gray!25}\vrule} 
}
    \arrayrulecolor{gray!25}\hline
    &
    \multicolumn{3}{ c !{\color{gray!25}\vrule} !{\color{gray!25}\vrule} }{Sum of Absolute Differences} & 
    \multicolumn{3}{ c !{\color{gray!25}\vrule} }{Mean Squared Error}
    \\
    \arrayrulecolor{gray!25}\hline
    &
    Overall &
    S &
    L &
    Overall &
    S &
    L
    \\
    Without CM & 
    -2.8 \% &
    -1.9 \% &
    -3.7 \% &
    -0.5 \% &
    -0.3 \% &
    -0.8 \% 
    \\
    Without \knt-\-to-\unt & 
    27.2 \% &
    14.6 \% &
    40.0 \% &
    27.8 \% &
    10.3 \% &
    45.2 \% 
    \\
    Without intra-\unt & 
    1.2 \% &
    1.2 \% &
    1.2 \% &
    7.2 \% &
    5.8 \% &
    8.6 \% 
    \\
    Without local & 
    4.4 \% &
    7.3 \% &
    1.5 \% &
    26.6 \% &
    30.6 \% &
    22.7 \% 
    \\
    \arrayrulecolor{gray!25}\hline
\end{tabular}
}
}
\label{tab:ablation}
\end{table}


==> images/benchmark.tex <==

\begin{table*}[t]
\caption{
Our scores in the alpha matting benchmark~\cite{alphabenchmark} together with the top-performing published methods at the time of submission.
\emph{S}, \emph{L} and \emph{U} denote the three trimap types, small, large and user, included in the benchmark.
Bold and blue numbers represent the best scores obtained among all the published methods in the benchmark$^*$.
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
\rowcolors{2}{gray!25}{}
\begin{tabular}{
     !{\color{gray!25}\vrule} 
     l 
     !{\color{gray!25}\vrule}
     c
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule} 
     c c c 
     !{\color{gray!25}\vrule}
     }
    \arrayrulecolor{gray!25}\hline
    &
    \multicolumn{4}{c !{\color{gray!25}\vrule} }{Average Rank$^{**}$} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Troll} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Doll} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Donkey} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Elephant} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Plant} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Pineapple} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Plastic bag} &
    \multicolumn{3}{c !{\color{gray!25}\vrule} }{Net}
    \\
    & 
    \emph{Overall} & 
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U} &
    \emph{S} &     \emph{L} &     \emph{U}
    \\
    %%%%% SAD %%%%%
    \arrayrulecolor{gray!25}\hline
 \multicolumn{29}{!{\color{gray!25}\vrule}c !{\color{gray!25}\vrule} }{Sum of Absolute Differences}\\
    \arrayrulecolor{gray!25}\hline
    %\rowcolor{gray!25}
    Ours & 2.1 & 2.8 & 1.6 & 2.0 & %2.7    & 3.3   & 2.3   & 2.6   &
    \topscore{10.3}  & \topscore{11.2}  & {12.5}  & 
    {5.6}  & {7.3}  & {7.3}  & 
    \topscore{3.8}  & \topscore{4.1}  & \topscore{3}  & 
    \topscore{1.4}  & \topscore{2.3}  & \topscore{2.0}  & 
    {5.9}  & {7.1}  & \topscore{8.6}  & 
    \topscore{3.6}  & \topscore{5.7}  & \topscore{4.6}  & 
    {18.3}  & {19.3}  & \topscore{15.8}  & 
    {20.2}  & {22.2}  & {22.3}
    \\
    DCNN \cite{dcnn} &  3.2 & 4.6 & 1.6 & 3.4 & %4.0   &  5.4  &  2.3  & 4.3   &
    {12.0}  & {14.1}  & {14.5}  & 
    \topscore{5.3}  & \topscore{6.4}  & {6.8}  & 
    {3.9}  & {4.5}  & {3.4}  & 
    {1.6}  & {2.5}  & {2.2}  & 
    {6.0}  & \topscore{6.9}  & {9.1}  & 
    {4.0}  & {6.0}  & {5.3}  & 
    {19.9}  & \topscore{19.2}  & {19.1}  & 
    \topscore{19.4}  & \topscore{20.0}  & \topscore{21.2}
    \\
    %\rowcolor{gray!25}
    CSC \cite{csc} &   10 & 13.5 & 6.4 & 10.3 & %11  &  14.4  &  7.4  &  11.3  &
    13.6 & 15.6 & 14.5 & 6.2 & 7.5 & 8.1 & 4.6 & 4.8 & 4.2 & 1.8 & 2.7 & 2.5 & 5.5 & 7.3 & 9.7 & 4.6 & 7.6 & 6.9 & 23.7 & 23.0 & 21.0 & 26.3 & 27.2 & 25.2
    \\
    LNSP \cite{lnsp} & 10.7 & 7.3 & 10.3 & 14.6 & %11.6    & 8.3   &   11.3 & 15.4   &
    12.2 & 22.5 & 19.5 & 5.6 & 8.1 & 8.8 & 4.6 & 5.9 & 3.6 & 1.5 & 3.5 & 3.1 & 6.2 & 8.1 & 10.7 & 4.0 & 7.1 & 6.4 & 21.5 & 20.8 & 16.3 & 22.5 & 24.4 & 27.8
    \\
    %%%%% MSE %%%%%
    \arrayrulecolor{gray!25}\hline
 \multicolumn{29}{!{\color{gray!25}\vrule}c !{\color{gray!25}\vrule} }{Mean Squared Error}\\
    \arrayrulecolor{gray!25}\hline
    %\rowcolor{gray!25}
    Ours & 
    3.5 &
    5.0 & 2.1 & 3.4 & 
    \topscore{0.3} & \topscore{0.4} & {0.5} & 
    {0.3} & {0.4} & {0.5} & 
    {0.3} & {0.3} & {0.2} & 
    {0.1} & {0.1} & {0.1} & 
    {0.4} & {0.4} & \topscore{0.6} & 
    {0.2} & \topscore{0.3} & {0.3} & 
    {1.3} & {1.2} & \topscore{0.8} & 
    {0.8} & {0.8} & {0.9}
    \\
    DCNN \cite{dcnn} &  
    3.7 &
    4.5 & 1.9 & 4.6 & 
    {0.4} & {0.5} & {0.7} & 
    \topscore{0.2} & \topscore{0.3} & {0.4} & 
    \topscore{0.2} & {0.3} & {0.2} & 
    {0.1} & \topscore{0.1} & \topscore{0.1} & 
    {0.4} & \topscore{0.4} & {0.8} & 
    {0.2} & {0.4} & {0.3} & 
    {1.3} & {1.2} & {1.0} & 
    \topscore{0.7} & \topscore{0.7} & {0.9}
    \\
    %\rowcolor{gray!25}
    LNSP \cite{lnsp} & 
    9.2 &
    6.6 & 8.6 & 12.4 &
    {0.5} & {1.9} & {1.2} & 
    {0.2} & {0.4} & {0.5} & 
    {0.3} & {0.4} & {0.2} & 
    \topscore{0.0} & {0.1} & {0.2} & 
    {0.4} & {0.5} & {0.8} & 
    \topscore{0.2} & {0.3} & {0.4} & 
    {1.4} & {1.2} & {0.8} & 
    {1.0} & {1.1} & {1.5}
    \\
    KL-D \cite{kldiv} & 
    11.6 &
    11.0 & 10.5 & 13.3 &
    {0.4} & {0.9} & {0.7} & 
    {0.3} & {0.5} & {0.5} & 
    {0.3} & {0.4} & {0.3} & 
    {0.1} & {0.2} & {0.1} & 
    {0.4} & {0.4} & {1.2} & 
    {0.4} & {0.6} & {0.6} & 
    {1.7} & {2.0} & {2.1} & 
    {0.8} & {0.8} & {0.9}
    \\
    \arrayrulecolor{gray!25}\hline
\rowcolor{white}
 \multicolumn{29}{ l }
 {$^*$ Some columns do not have a bold number when the best-scoring algorithm for that particular image-trimap pair is not among the top-ranking methods included here.}
 \\
\rowcolor{white}
 \multicolumn{29}{ l }
 {$^{**}$ The ranks presented here only take the already-published methods at the time of the submission into account, hence could differ from the online version of the benchmark.}
\end{tabular}}
}
\label{tab:benchmark}
\end{table*}






==> imagetex/AlphaColorTest2.tex <==
\begin{figure*}
\centering
{
\showimagew[0.95\linewidth]{images/AlphaColorComp_Donkey.jpg}
}
\caption{
Different pairings of alpha and color estimation methods. Best seen in the digital version. See text for discussion.
\negvspace
\negvspace
\negvspace
\negvspace
}
\label{fig:alphacolordonkey}
\end{figure*}


==> imagetex/AlphaColorTest8.tex <==
\begin{figure}
\showimagew[\linewidth]{images/AlphaColorComp_Troll_OneColumn.jpg}
\caption{
Different pairings of alpha and color estimation methods. Best seen in the digital version. See text for discussion.
}
\negvspace
\negvspace
\negvspace
\label{fig:alphacolortroll}
\end{figure}


==> imagetex/DIMDatasetRes.tex <==
\begin{figure}
{
\footnotesize
\begin{tabular}
{   K{0.285\linewidth}
    K{0.285\linewidth}
    K{0.285\linewidth}
}
Input and trimap&
Our result&
Ground truth
\end{tabular}
}
\showimagew[\linewidth]{images/DIMDatasetRes.jpg}
\caption{
Example results from the deep image matting test dataset~\cite{deepmatting} with trimaps shown with the input image.
}
\negvspace
\label{fig:DIMDatasetRes}
\end{figure}


==> imagetex/GreenScreenKeying2.tex <==
\begin{figure}[t]
%\showimagew[\linewidth]{images/GreenScreenKeying_Scientist.jpg}
%\vspace{0.01cm}\\
\showimagew[\linewidth]{images/GreenScreenKeying_AmitVertical.jpg}
\caption{
Green-screen keying results of GSK~\cite{keying} with its input called
\emph{local color models} (a) and of SCS~\cite{softcolorsegm} with the mask
needed for a clean result (b) together with the proposed method (c),
comprehensive sampling~\cite{comprehensive} (d) and KNN matting~\cite{knnpami} (e)
using two trimaps, one narrow and one wide, for each example.
See text for discussion.
}
\negvspace
\label{fig:keying2}
\end{figure}


==> imagetex/Spectral_Training4.tex <==
\begin{figure*}[b]
{
\footnotesize
\begin{tabular}
{   K{0.143\linewidth}
    K{0.143\linewidth}
    K{0.143\linewidth}
    K{0.143\linewidth}
    K{0.143\linewidth}
    K{0.143\linewidth}
}
Input&
Only CM&
Only intra-\unt&
Only local&
CM \& intra-\unt&
CM, intra-\unt\ \& local
\end{tabular}
}
\showimagew[\linewidth]{images/Spectral_Training4.jpg}
\caption{
Matting components \cite{spectralpami} corresponding to the pink and the green hair using Laplacian matrices constructed using different subsets of information flow.
See text for discussion.
}
\label{fig:spectral4}
\end{figure*}


==> imagetex/teaser.tex <==
\begin{figure*}[h]
\showimagew[\linewidth]{images/teaser4DoubleColumn.jpg}
\caption{
For an input image and a trimap (a), we construct our linear system by first using the color-mixture flow(b), then adding direct channels of information flow from known to unknown regions (c), and letting information be shared effectively inside the unknown region (d).
We finally introduce local information flow to enforce spatial smoothness (e).
Note that the intermediate results in this figure are solely for illustration.
In practice, we construct a single energy function that accounts for all types of information flow and solve it once to obtain the end result.
}
\negvspace
\negvspace
\label{fig:teaser}
\end{figure*}

